Workload Intelligence: Punching Holes Through the Cloud Abstraction

Today, cloud workloads are essentially opaque to the cloud platform. Typically, the only information the platform receives is the virtual machine (VM) type and possibly a decoration to the type (e.g., the VM is evictable). Similarly, workloads receive little to no information from the platform; generally, workloads might receive telemetry from their VMs or exceptional signals (e.g., shortly before a VM is evicted). The narrow interface between workloads and platforms has several drawbacks: (1) a surge in VM types and decorations in public cloud platforms complicates customer selection; (2) essential workload characteristics (e.g., low availability requirements, high latency tolerance) are often unspecified, hindering platform customization for optimized resource usage and cost savings; and (3) workloads may be unaware of potential optimizations or lack sufficient time to react to platform events. In this paper, we propose a framework, called Workload Intelligence (WI), for dynamic bi-directional communication between cloud workloads and cloud platform. Via WI, workloads can programmatically adjust their key characteristics, requirements, and even dynamically adapt behaviors like VM priorities. In the other direction, WI allows the platform to programmatically inform workloads about upcoming events, opportunities for optimization, among other scenarios. Because of WI, the cloud platform can drastically simplify its offerings, reduce its costs without fear of violating any workload requirements, and reduce prices to its customers on average by 48.8%.

==> experimental.tex <==

\section{Experimental setup}
\subsection{Extending systems}
\begin{itemize}
    \item Focus: Multiple workloads can benefit from one system
    \item Workload 1: Terasort/Teragen running on Hadoop
    \item Workload 2: Teams video conferencing
\end{itemize}

\subsubsection{Multi-availability system}
\begin{itemize}
    \item Workload: Teams and Hadoop
    \item Mechanism: When an incident event happens, we throttle the the VMs of lower required availability and/or evict the VMs that are preemptible.
    \item Metrics: Data centers' (DC) cost 
\end{itemize}

\subsubsection{Harvest VMs}
\begin{itemize}
    \item Workload: Hadoop
    \item Shrink/Expand/Evict Harvest VMs depending on available resources left
    \item Metrics: DC cost
\end{itemize}

\subsubsection{Overclocking}
\begin{itemize}
    \item Workload: Teams
    \item For air-cooling system, depending on the thermos budget, we overclock at different frequencies
    \item For liquid-cooling system, depending on the reliability budget, we overclock at different frequencies
    \item Metrics: DC cost
\end{itemize}

\subsubsection{Underclocking}
\begin{itemize}
    \item Workload: Teams
    \item Considering the source of the energy usage, the cloud platform can underclock when using non-sustainable energy and overclock to speed up the workload processing when using green energy.
    \item Metrics: Carbon footprint
\end{itemize}

\subsubsection{Oversubscription (CPU, Memory, Power)}
\begin{itemize}
    \item Workload: Teams? and/or SocialNetwork
    \item Mechanisms: 
    \item Metrics: DC cost
\end{itemize}

\subsubsection{Auto-scaling}
\begin{itemize}
    \item Workload: Hadoop
    \item Launch more VMs to process the workload if resources available
    \item Metrics: DC cost
\end{itemize}

\subsubsection{Resource Prioritization Service}
\begin{itemize}
    \item Workload: Teams and Hadoop
    \item Based on the workload priorities, the cloud platform deploys new VMs with different time constraints
    \item Metrics: Charged based on (saved launching time * price per VM)
    \item Contact Randolph for VM launching times
\end{itemize}

\subsubsection{Region-Agnostic placement}
\begin{itemize}
    \item Workload: SocialNetwork
    \item Based on the cloud DC utilization, the cloud platform balance the load across the DCs by placing VMs differently.
    \item Metrics: DC cost
\end{itemize}






